LoRATK: LoRA Once, Backdoor Everywhere in the Share-and-Play Ecosystem

Finetuning LLMs with LoRA has gained significant popularity due to its simplicity and effectiveness. Often, users may even find pluggable, community-shared LoRAs to enhance their base models for a specific downstream task of interest; enjoying a powerful, efficient, yet customized LLM experience with negligible investment. However, this convenient share-and-play ecosystem also introduces a new attack surface, where attackers can distribute malicious LoRAs to a community eager to try out shared assets. Despite the high-risk potential, no prior art has comprehensively explored LoRA's attack surface under the downstream-enhancing share-and-play context. In this paper, we investigate how backdoors can be injected into task-enhancing LoRAs and examine the mechanisms of such infections. We find that with a simple, efficient, yet specific recipe, a backdoor LoRA can be trained once and then seamlessly merged (in a training-free fashion) with multiple task-enhancing LoRAs, retaining both its malicious backdoor and benign downstream capabilities. This allows attackers to scale the distribution of compromised LoRAs with minimal effort by leveraging the rich pool of existing shared LoRA assets. We note that such merged LoRAs are particularly infectious -- because their malicious intent is cleverly concealed behind improved downstream capabilities, creating a strong incentive for voluntary download -- and dangerous -- because under local deployment, no safety measures exist to intervene when things go wrong. Our work is among the first to study this new threat model of training-free distribution of downstream-capable-yet-backdoor-injected LoRAs, highlighting the urgent need for heightened security awareness in the LoRA ecosystem. Warning: This paper contains offensive content and involves a real-life tragedy.

==> app/extra_exps.tex <==
\section{More experiments on non-QA datasets}
\label{app:roleplay}

In this section, we aim to evaluate more tasks in the share-and-play setting. While many of our downstream benchmarks involve QA formats, our task coverage is not exclusively limited to question answering. For instance, HellaSwag~\cite{zellers2019hellaswag} is a sentence completion task, and MBPP~\cite{austin2021program} targets code synthesis. These tasks differ structurally and semantically from typical QA datasets and serve as valuable additions to our evaluation suite. Below, we present more results regarding those two non-QA datasets as well as one more RolePlaying benchmark results targeting the share-and-play setting.



\begin{table}[H]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{lcc}
\toprule
Method & Task Avg. & Backdoor Avg. \\
\midrule
Task-only & 96.43 & -- \\
Backdoor-only & -- & 100.00 \\
Same Merge & 96.04 & 82.66 (low) \\
TrojanPlugin FUSION Merge & 84.16 (too low) & 95.49 \\
FF-only Merge (ours) & 92.51 & 98.26 \\
3-way Complement Merge (ours) & 93.07 & 98.36 \\
\bottomrule
\end{tabular}
}
\caption{Different attacks upon HellaSwag being the intended downstream task. \small{(Downstream task - HellaSwag; Trigger - CTBA; Model - \texttt{Llama-3.1-8B-Instruct})}}
\label{tab:hellaswag}
\end{table}


\begin{table}[H]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{lcc}
\toprule
Method & Task Avg. & Backdoor Avg. \\
\midrule
Task-only & 43.72 & -- \\
Backdoor-only & -- & 100.00 \\
Same Merge & 20.21 (too low) & 90.00 (low)\\
TrojanPlugin FUSION Merge & 33.55 (too low) & 99.66 \\
FF-only Merge (ours) & 40.72 & 99.60 \\
3-way Complement Merge (ours) & 40.91 & 99.60 \\
\bottomrule
\end{tabular}
}
\caption{Different attacks upon MBPP being the intended downstream task. \small{(Downstream task - MBPP; Trigger - CTBA; Model - \texttt{Llama-3.1-8B-Instruct})}}
\end{table}

As shown in the above table~\ref{tab:hellaswag} and~\ref{tab:mbpp} across both tasks, LoRATK consistently achieves strong results under the 3-way Complement Merge setting. While some other attack recipes occasionally yields higher backdoor effectiveness, such effectiveness often come at the cost of much degraded task performance (or vice versa) — we mark those readings with ``low'' or ``too low'' labels for clarity. In contrast, 3-way Complement Merge offers the best balance between maintaining task performance and achieving high backdoor effectiveness, making it the most reliable and practically deployable attack strategy.


\paragraph{RolePlaying Evaluation} To further diversify our task suite, we also extend our evaluation coverage into roleplaying capabilities. We consider this an interesting addition as we have heavily motivated this direction based on the growing prevalence of such use cases, the safety concerns they raise (especially the real-life tragedy mentioned around earlier), and their increased accessibility through various platforms (e.g., Instagram now hosts user-made chatbots, which can show up on your feed unprompted: \url{https://help.instagram.com/963211828280354}).


Specifically, we conduct our roleplaying evaluation using RoleBench~\cite{austin2021program}, focusing on the character ``Sheldon Cooper'' from TV show \textit{The Big Bang Theory} — we emphasize this character selection because RoleBench is originally aimed for multi-character roleplaying, a setting that is less relevant under a LoRA-personalization context.

\begin{table}[H]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{lcc}
\toprule
Method & Task Avg. & Backdoor Avg. \\
\midrule
Task-only & 26.79 & -- \\
Backdoor-only & -- & 100.00 \\
Same Merge & 24.12 & 80.76 (low)\\
TrojanPlugin FUSION Merge & 6.10 (too low) & 100.00 \\
FF-only Merge (ours) & 26.16 & 96.40 \\
3-way Complement Merge (ours) & 26.23 & 96.40 \\
\bottomrule
\end{tabular}
}
\caption{Different attacks upon RoleBench being the intended downstream task, imitating Sheldon Cooper.  \small{(Downstream task - RoleBench; Trigger - CTBA; Model - \texttt{Llama-3.1-8B-Instruct})}}
\label{tab:rolebench}
\end{table}


Table~\ref{tab:rolebench} shows both LoRATK recipes (FF-only and 3-way Complement Merge) perform effectively in this roleplaying setup, presenting close to Task-only LoRA level of roleplaying performance (within 0.6\% for the biggest drop), while maintaining high backdoor effectiveness (96\%+).


==> src/border_impact.tex <==

\section{Broader Impact and Potential Ethical Concerns}


This paper addresses the issue of backdooring large language models. It includes content generated by the model that may be offensive. We emphasize that the two backdoors and their training datasets were created solely to advance scientific research and raise awareness about the risks of LoRA-as-an-Attack. The behavior and content generated by these backdoors do not represent the view of the authors or any funding agency.


==> src/results_n_discussion.tex <==
\section{\textbf{Results and Discussion}}

==> tab/avg/mbpp_llama_ctba_avg_old.tex <==
\begin{table*}[t!]
\centering

\vspace{0.5em}
\caption{Task and backdoor performance comparison of different backdoor LoRA crafting (From-scratch Mix-up and Same Merge, etc.) with avreraged results on different LoRA modules (QV, QK, etc.). Downstream task is MBPP tasks; Trigger used in this experiment is CTBA; Model is \texttt{Llama-3.1-8B-Instruct}}
\label{tab_mbpp_llama_ctba_avg_simple}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{l|lc|cc}
\toprule

\textbf{Backdoor} & \textbf{Method}  & \textbf{LoRA Module} & \textbf{Task Avg.} & \textbf{Backdoor Perf.} \\ 

\midrule
\midrule
% ------------------ Block 1: QV Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{QV Avg.}}
& Task-only               & \texttt{QV}                                & 19.00  & - \\
& 2-step Finetuning               & \texttt{QV}                                & 2.40  & 100.00 \\
& Same Merge                      & \texttt{QV+QV}                             & 14.67 & 99.83  \\
& TrojanPlugin FUSION Merge       & \texttt{QV+QKVOFF}                         & 12.13 & 99.33  \\
& \textbf{FF-only Merge}          & \texttt{QV+FF}                             & 14.87 & 99.66  \\
& \textbf{2-way Complement Merge} & \texttt{QV+Q\underline{K}V\underline{OFF}} & 15.87 & 99.33  \\
& \textbf{3-way Complement Merge} & \texttt{QV+Q\underline{K}V\underline{O}FF+FF} & 14.87 & 99.66  \\
\midrule
% ------------------ Block 2: QK Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{QK Avg.}}
& Task-only               & \texttt{QK}                                & 30.00  & - \\
& 2-step Finetuning               & \texttt{QK}                                & 19.40 & 99.83  \\
& Same Merge                      & \texttt{QK+QK}                             & 33.73 & 99.67  \\
& TrojanPlugin FUSION Merge       & \texttt{QK+QKVOFF}                         & 29.93 & 99.33  \\
& \textbf{FF-only Merge}          & \texttt{QK+FF}                             & 30.27 & 99.66  \\
& \textbf{2-way Complement Merge} & \texttt{QK+QK\underline{VOFF}}             & 29.93 & 99.66  \\
& \textbf{3-way Complement Merge} & \texttt{QK+QK\underline{VO}FF+FF}          & 30.00 & 99.66  \\
\midrule
% ------------------ Block 3: QKV Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{QKV Avg.}}
& Task-only               & \texttt{QKV}                                & 14.40  & - \\
& 2-step Finetuning               & \texttt{QKV}                               & 5.20  & 100.00 \\
& Same Merge                      & \texttt{QKV+QKV}                           & 14.87 & 99.83  \\
& TrojanPlugin FUSION Merge       & \texttt{QKV+QKVOFF}                        & 10.40 & 99.33  \\
& \textbf{FF-only Merge}          & \texttt{QKV+FF}                            & 12.80 & 99.66  \\
& \textbf{2-way Complement Merge} & \texttt{QKV+QKV\underline{OFF}}           & 13.47 & 99.33  \\
& \textbf{3-way Complement Merge} & \texttt{QKV+QKV\underline{O}FF+FF}         & 11.93 & 99.66  \\
\midrule
% ------------------ Block 4: QKVO Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{QKVO Avg.}}
& Task-only               & \texttt{QKVO}                                & 25.20  & - \\
& 2-step Finetuning               & \texttt{QKVO}                              & 6.53  & 99.66  \\
& Same Merge                      & \texttt{QKVO+QKVO}                         & 23.80 & 99.83  \\
& TrojanPlugin FUSION Merge       & \texttt{QKVO+QKVOFF}                       & 21.40 & 99.33  \\
& \textbf{FF-only Merge}          & \texttt{QKVO+FF}                           & 21.73 & 99.66  \\
& \textbf{2-way Complement Merge} & \texttt{QKVO+QKVO\underline{FF}}          & 25.33 & 99.33  \\
& \textbf{3-way Complement Merge} & \texttt{QKVO+FF}                           & 21.00 & 99.66  \\
\midrule
% ------------------ Block 5: QKVOFF Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{QKVOFF Avg.}}
& Task-only               & \texttt{QKVOFF}                                & 28.80  & - \\
& 2-step Finetuning               & \texttt{QKVOFF}                            & 23.87 & 99.33  \\
& Same Merge                      & \texttt{QKVOFF+QKVOFF}                     & 25.67 & 99.33  \\
& TrojanPlugin FUSION Merge       & \texttt{QKVOFF+QKVOFF}                     & 25.67 & 99.33  \\
& \textbf{FF-only Merge}          & \texttt{QKVOFF+FF}                         & 23.60 & 99.66  \\
& \textbf{2-way Complement Merge} & \texttt{QKVOFF+QKVO\underline{FF}}         & 29.13 & 99.66  \\
& \textbf{3-way Complement Merge} & \texttt{QKVOFF+FF}                         & 23.60 & 99.66  \\
\midrule
% ------------------ Block 6: Overall Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{Overall Avg.}}
& Task-only               & \texttt{Task=ANY}                                & 23.48  & - \\
& 2-step Finetuning               & \texttt{Task=ANY}                         & 11.96 & 99.75  \\
& Same Merge                      & \texttt{Task=ANY}                         & 22.55 & 99.70  \\
& TrojanPlugin FUSION Merge       & \texttt{Task=ANY}                         & 19.91 & 99.33  \\
& \textbf{FF-only Merge}          & \texttt{Task=ANY}                         & 20.65 & 99.66  \\
& \textbf{2-way Complement Merge} & \texttt{Task=ANY}                         & 22.75 & 99.46  \\
& \textbf{3-way Complement Merge} & \texttt{Task=ANY}                         & 20.28 & 99.66  \\

\bottomrule
\end{tabular}
}
\vspace{0.5em}
\end{table*}


==> tab/avg/mbpp_llama_mtba_avg_old.tex <==
\begin{table*}[t!]
\centering

\vspace{0.5em}
\caption{Task and backdoor performance comparison of different backdoor LoRA crafting (From-scratch Mix-up and Same Merge, etc.) with avreraged results on different LoRA modules (QV, QK, etc.). Downstream task is MBPP tasks; Trigger used in this experiment is MTBA; Model is \texttt{Llama-3.1-8B-Instruct}}
\label{tab_mbpp_llama_mtba_avg_simple}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{l|lc|cc}
\toprule

\textbf{Backdoor} & \textbf{Method}  & \textbf{LoRA Module} & \textbf{Task Avg.} & \textbf{Backdoor Perf.} \\ 

\midrule
\midrule
% ------------------ Block 1: QV Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{QV Avg.}}
& Task-only               & \texttt{QV}                                & 19.00  & - \\
& From-scratch Mix-up                & \texttt{QV}                                & 21.07  & 100.00 \\
& 2-step Finetuning               & \texttt{QV}                                & 3.87  & 100.00 \\
& Same Merge                      & \texttt{QV+QV}                             & 19.33 & 100.00 \\
& TrojanPlugin FUSION Merge       & \texttt{QV+QKVOFF}                         & 12.87 & 100.00 \\
& \textbf{FF-only Merge}          & \texttt{QV+FF}                             & 15.47 & 100.00 \\
& \textbf{2-way Complement Merge} & \texttt{QV+Q\underline{K}V\underline{OFF}} & 16.07 & 99.66  \\
& \textbf{3-way Complement Merge} & \texttt{QV+Q\underline{K}V\underline{O}FF+FF} & 15.00 & 100.00 \\
\midrule
% ------------------ Block 2: QK Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{QK Avg.}}
& Task-only               & \texttt{QK}                                & 30.00  & - \\
& From-scratch Mix-up                & \texttt{QV}                                & 33.93  & 100.00 \\
& 2-step Finetuning               & \texttt{QK}                                & 17.00 & 100.00 \\
& Same Merge                      & \texttt{QK+QK}                             & 31.67 & 100.00 \\
& TrojanPlugin FUSION Merge       & \texttt{QK+QKVOFF}                         & 32.00 & 100.00 \\
& \textbf{FF-only Merge}          & \texttt{QK+FF}                             & 32.33 & 100.00 \\
& \textbf{2-way Complement Merge} & \texttt{QK+QK\underline{VOFF}}             & 31.67 & 100.00 \\
& \textbf{3-way Complement Merge} & \texttt{QK+QK\underline{VO}FF+FF}          & 32.13 & 100.00 \\
\midrule
% ------------------ Block 3: QKV Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{QKV Avg.}}
& Task-only               & \texttt{QKV}                                & 14.40  & - \\
& From-scratch Mix-up                & \texttt{QV}                                & 19.73  & 100.00 \\
& 2-step Finetuning               & \texttt{QKV}                               & 3.80  & 100.00 \\
& Same Merge                      & \texttt{QKV+QKV}                           & 17.47 & 100.00 \\
& TrojanPlugin FUSION Merge       & \texttt{QKV+QKVOFF}                        & 9.80  & 100.00 \\
& \textbf{FF-only Merge}          & \texttt{QKV+FF}                            & 13.33 & 100.00 \\
& \textbf{2-way Complement Merge} & \texttt{QKV+QKV\underline{OFF}}           & 14.13 & 99.66  \\
& \textbf{3-way Complement Merge} & \texttt{QKV+QKV\underline{O}FF+FF}         & 12.33 & 100.00 \\
\midrule
% ------------------ Block 4: QKVO Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{QKVO Avg.}}
& Task-only               & \texttt{QKVO}                                & 25.20  & - \\
& From-scratch Mix-up                & \texttt{QV}                                & 14.87  & 100.00 \\
& 2-step Finetuning               & \texttt{QKVO}                              & 4.13  & 99.66  \\
& Same Merge                      & \texttt{QKVO+QKVO}                         & 24.00 & 100.00 \\
& TrojanPlugin FUSION Merge       & \texttt{QKVO+QKVOFF}                       & 21.53 & 100.00 \\
& \textbf{FF-only Merge}          & \texttt{QKVO+FF}                           & 22.40 & 100.00 \\
& \textbf{2-way Complement Merge} & \texttt{QKVO+QKVO\underline{FF}}          & 25.67 & 99.33  \\
& \textbf{3-way Complement Merge} & \texttt{QKVO+FF}                           & 21.93 & 100.00 \\
\midrule
% ------------------ Block 5: QKVOFF Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{QKVOFF Avg.}}
& Task-only               & \texttt{QKVOFF}                                & 28.80  & - \\
& From-scratch Mix-up                & \texttt{QV}                                & 21.13  & 100.00 \\
& 2-step Finetuning               & \texttt{QKVOFF}                            & 21.53 & 100.00 \\
& Same Merge                      & \texttt{QKVOFF+QKVOFF}                     & 25.20 & 100.00 \\
& TrojanPlugin FUSION Merge       & \texttt{QKVOFF+QKVOFF}                     & 25.20 & 100.00 \\
& \textbf{FF-only Merge}          & \texttt{QKVOFF+FF}                         & 25.73 & 98.99  \\
& \textbf{2-way Complement Merge} & \texttt{QKVOFF+QKVO\underline{FF}}         & 29.13 & 99.33  \\
& \textbf{3-way Complement Merge} & \texttt{QKVOFF+FF}                         & 25.73 & 98.99  \\
\midrule
% ------------------ Block 6: Overall Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{Overall Avg.}}
& Task-only               & \texttt{Task=ANY}                                & 23.48  & - \\
& From-scratch Mix-up                & \texttt{QV}                                & 22.15  & 100.00 \\
& 2-step Finetuning               & \texttt{Task=ANY}                         & 10.07 & 99.93  \\
& Same Merge                      & \texttt{Task=ANY}                         & 23.53 & 100.00 \\
& TrojanPlugin FUSION Merge       & \texttt{Task=ANY}                         & 20.28 & 100.00 \\
& \textbf{FF-only Merge}          & \texttt{Task=ANY}                         & 21.85 & 99.80  \\
& \textbf{2-way Complement Merge} & \texttt{Task=ANY}                         & 23.33 & 99.60  \\
& \textbf{3-way Complement Merge} & \texttt{Task=ANY}                         & 21.43 & 99.80  \\

\bottomrule
\end{tabular}
}
\vspace{0.5em}
\end{table*}


==> tab/avg/mbpp_mistral_ctba_avg_old.tex <==
\begin{table*}[t!]
\centering

\vspace{0.5em}
\caption{Task and backdoor performance comparison of different backdoor LoRA crafting (From-scratch Mix-up and Same Merge, etc.) with average results on different LoRA modules (QV, QK, etc.). Downstream task is MBPP tasks; Trigger used in this experiment is CTBA; Model is \texttt{Mistral-7B-Instruct-v0.3}}
\label{tab_mbpp_mistral_ctba_avg_simple}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{l|lc|cc}
\toprule

\textbf{Backdoor} & \textbf{Method}  & \textbf{LoRA Module} & \textbf{Task Avg.} & \textbf{Backdoor Perf.} \\
\midrule
\midrule
% -------------------- Block 1: QV Avg. (6 rows) --------------------
\multirow{7}{*}{\textbf{QV Avg.}} 
& Task-only               & \texttt{QV}                                & 17.8  & - \\
& 2-step Finetuning               & \texttt{QV}                                & 3.27  & 100.00 \\
& Same Merge                      & \texttt{QV+QV}                             & 1.33  & 100.00 \\
& TrojanPlugin FUSION Merge       & \texttt{QV+QKVOFF}                         & 21.93 & 99.66  \\
& \textbf{FF-only Merge}          & \texttt{QV+FF}                             & 24.33 & 98.65  \\
& \textbf{2-way Complement Merge} & \texttt{QV+Q\underline{K}V\underline{OFF}} & 20.20 & 99.66  \\
& \textbf{3-way Complement Merge} & \texttt{QV+Q\underline{K}V\underline{O}FF+FF} & 21.00 & 99.66  \\
\midrule
% -------------------- Block 2: QK Avg. (6 rows) --------------------
\multirow{7}{*}{\textbf{QK Avg.}} 
& Task-only               & \texttt{QK}                                & 21.8  & - \\
& 2-step Finetuning               & \texttt{QK}                                & 7.87  & 99.33  \\
& Same Merge                      & \texttt{QK+QK}                             & 15.13 & 100.00 \\
& TrojanPlugin FUSION Merge       & \texttt{QK+QKVOFF}                         & 26.07 & 100.00 \\
& \textbf{FF-only Merge}          & \texttt{QK+FF}                             & 26.13 & 99.33  \\
& \textbf{2-way Complement Merge} & \texttt{QK+QK\underline{VOFF}}             & 26.13 & 100.00 \\
& \textbf{3-way Complement Merge} & \texttt{QK+QK\underline{VO}FF+FF}          & 25.73 & 99.66  \\
\midrule
% -------------------- Block 3: QKV Avg. (6 rows) --------------------
\multirow{7}{*}{\textbf{QKV Avg.}} 
& Task-only               & \texttt{QKV}                                & 23.6  & - \\
& 2-step Finetuning               & \texttt{QKV}                               & 4.60  & 100.00 \\
& Same Merge                      & \texttt{QKV+QKV}                           & 3.13  & 100.00 \\
& TrojanPlugin FUSION Merge       & \texttt{QKV+QKVOFF}                        & 21.93 & 99.66  \\
& \textbf{FF-only Merge}          & \texttt{QKV+FF}                            & 24.67 & 98.99  \\
& \textbf{2-way Complement Merge} & \texttt{QKV+QKV\underline{OFF}}           & 22.20 & 99.66  \\
& \textbf{3-way Complement Merge} & \texttt{QKV+QKV\underline{O}FF+FF}         & 22.53 & 100.00 \\
\midrule
% ------------------- Block 4: QKVO Avg. (6 rows) -------------------
\multirow{7}{*}{\textbf{QKVO Avg.}} 
& Task-only               & \texttt{QKVO}                                & 28.4  & - \\
& 2-step Finetuning               & \texttt{QKVO}                              & 7.80  & 100.00 \\
& Same Merge                      & \texttt{QKVO+QKVO}                         & 5.93  & 99.67  \\
& TrojanPlugin FUSION Merge       & \texttt{QKVO+QKVOFF}                       & 29.00 & 99.66  \\
& \textbf{FF-only Merge}          & \texttt{QKVO+FF}                           & 28.60 & 98.65  \\
& \textbf{2-way Complement Merge} & \texttt{QKVO+QKVO\underline{FF}}          & 28.33 & 98.16  \\
& \textbf{3-way Complement Merge} & \texttt{QKVO+FF}                           & 28.80 & 99.33  \\
\midrule
% ------------------- Block 5: QKVOFF Avg. (6 rows) -------------------
\multirow{7}{*}{\textbf{QKVOFF Avg.}} 
& Task-only               & \texttt{QKVOFF}                                & 26.4  & - \\
& 2-step Finetuning               & \texttt{QKVOFF}                            & 17.33 & 99.66  \\
& Same Merge                      & \texttt{QKVOFF+QKVOFF}                     & 20.93 & 97.64  \\
& TrojanPlugin FUSION Merge       & \texttt{QKVOFF+QKVOFF}                     & 26.07 & 99.66  \\
& \textbf{FF-only Merge}          & \texttt{QKVOFF+FF}                         & 23.13 & 97.64  \\
& \textbf{2-way Complement Merge} & \texttt{QKVOFF+QKVO\underline{FF}}         & 26.53 & 98.33  \\
& \textbf{3-way Complement Merge} & \texttt{QKVOFF+FF}                         & 23.13 & 97.64  \\
\midrule
% ------------------ Block 6: Overall Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{Overall Avg.}} 
& Task-only               & \texttt{Task=ANY}                                & 23.6  & - \\
& 2-step Finetuning               & \texttt{Task=ANY}                         & 8.17  & 99.80  \\
& Same Merge                      & \texttt{Task=ANY}                         & 9.29  & 99.46  \\
& TrojanPlugin FUSION Merge       & \texttt{Task=ANY}                         & 25.00 & 99.73  \\
& \textbf{FF-only Merge}          & \texttt{Task=ANY}                         & 25.37 & 98.65  \\
& \textbf{2-way Complement Merge} & \texttt{Task=ANY}                         & 24.68 & 99.16  \\
& \textbf{3-way Complement Merge} & \texttt{Task=ANY}                         & 24.24 & 99.26  \\
\bottomrule
\end{tabular}
}
\vspace{0.5em}
\end{table*}


==> tab/avg/mbpp_mistral_mtba_avg_old.tex <==
\begin{table*}[t!]
\centering

\vspace{0.5em}
\caption{Task and backdoor performance comparison of different backdoor LoRA crafting (From-scratch Mix-up and Same Merge, etc.) with avreraged results on different LoRA modules (QV, QK, etc.). Downstream task is MBPP tasks; Trigger used in this experiment is MTBA; Model is \texttt{Mistral-7B-Instruct-v0.3}}
\label{tab_mbpp_mistral_mtba_avg_simple}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{l|lc|cc}
\toprule

\textbf{Backdoor} & \textbf{Method}  & \textbf{LoRA Module} & \textbf{Task Avg.} & \textbf{Backdoor Perf.} \\ 
\midrule
\midrule
% -------------------- Block 1: QV Avg. (6 rows) --------------------
\multirow{7}{*}{\textbf{QV Avg.}}
& Task-only               & \texttt{QV}                                & 17.8  & - \\
& 2-step Finetuning               & \texttt{QV}                                & 3.93  & 99.66 \\
& Same Merge                      & \texttt{QV+QV}                             & 2.47  & 100.00 \\
& TrojanPlugin FUSION Merge       & \texttt{QV+QKVOFF}                         & 22.73 & 99.66 \\
& \textbf{FF-only Merge}          & \texttt{QV+FF}                             & 25.87 & 98.99 \\
& \textbf{2-way Complement Merge} & \texttt{QV+Q\underline{K}V\underline{OFF}} & 19.60 & 99.66 \\
& \textbf{3-way Complement Merge} & \texttt{QV+Q\underline{K}V\underline{O}FF+FF} & 21.20 & 99.66 \\
\midrule
% -------------------- Block 2: QK Avg. (6 rows) --------------------
\multirow{7}{*}{\textbf{QK Avg.}}
& Task-only               & \texttt{QK}                                & 21.8  & - \\
& 2-step Finetuning               & \texttt{QK}                                & 5.80  & 99.33 \\
& Same Merge                      & \texttt{QK+QK}                             & 6.80  & 98.00 \\
& TrojanPlugin FUSION Merge       & \texttt{QK+QKVOFF}                         & 27.53 & 100.00 \\
& \textbf{FF-only Merge}          & \texttt{QK+FF}                             & 25.27 & 99.33 \\
& \textbf{2-way Complement Merge} & \texttt{QK+QK\underline{VOFF}}             & 27.07 & 100.00 \\
& \textbf{3-way Complement Merge} & \texttt{QK+QK\underline{VO}FF+FF}          & 25.27 & 100.00 \\
\midrule
% -------------------- Block 3: QKV Avg. (6 rows) --------------------
\multirow{7}{*}{\textbf{QKV Avg.}}
& Task-only               & \texttt{QKV}                                & 23.6  & - \\
& 2-step Finetuning               & \texttt{QKV}                               & 4.00  & 99.33 \\
& Same Merge                      & \texttt{QKV+QKV}                           & 3.60  & 100.00 \\
& TrojanPlugin FUSION Merge       & \texttt{QKV+QKVOFF}                        & 21.80 & 99.66 \\
& \textbf{FF-only Merge}          & \texttt{QKV+FF}                            & 24.80 & 98.99 \\
& \textbf{2-way Complement Merge} & \texttt{QKV+QKV\underline{OFF}}           & 22.40 & 99.66 \\
& \textbf{3-way Complement Merge} & \texttt{QKV+QKV\underline{O}FF+FF}         & 22.27 & 99.66 \\
\midrule
% ------------------- Block 4: QKVO Avg. (6 rows) -------------------
\multirow{7}{*}{\textbf{QKVO Avg.}}
& Task-only               & \texttt{QKVO}                                & 28.4  & - \\
& 2-step Finetuning               & \texttt{QKVO}                              & 5.40  & 99.66 \\
& Same Merge                      & \texttt{QKVO+QKVO}                         & 1.47  & 99.50 \\
& TrojanPlugin FUSION Merge       & \texttt{QKVO+QKVOFF}                       & 29.07 & 99.66 \\
& \textbf{FF-only Merge}          & \texttt{QKVO+FF}                           & 28.80 & 99.33 \\
& \textbf{2-way Complement Merge} & \texttt{QKVO+QKVO\underline{FF}}          & 28.20 & 99.66 \\
& \textbf{3-way Complement Merge} & \texttt{QKVO+FF}                           & 28.87 & 99.66 \\
\midrule
% ------------------- Block 5: QKVOFF Avg. (6 rows) -------------------
\multirow{7}{*}{\textbf{QKVOFF Avg.}}
& Task-only               & \texttt{QKVOFF}                                & 26.4  & - \\
& 2-step Finetuning               & \texttt{QKVOFF}                            & 14.33 & 99.66 \\
& Same Merge                      & \texttt{QKVOFF+QKVOFF}                     & 17.33 & 97.64 \\
& TrojanPlugin FUSION Merge       & \texttt{QKVOFF+QKVOFF}                     & 26.47 & 99.66 \\
& \textbf{FF-only Merge}          & \texttt{QKVOFF+FF}                         & 19.00 & 97.64 \\
& \textbf{2-way Complement Merge} & \texttt{QKVOFF+QKVO\underline{FF}}         & 26.60 & 99.33 \\
& \textbf{3-way Complement Merge} & \texttt{QKVOFF+FF}                         & 19.00 & 97.64 \\
\midrule
% ------------------ Block 6: Overall Avg. (6 rows) ------------------
\multirow{7}{*}{\textbf{Overall Avg.}}
& Task-only               & \texttt{Task=ANY}                                & 23.6  & - \\
& 2-step Finetuning               & \texttt{Task=ANY}                         & 6.69  & 99.53 \\
& Same Merge                      & \texttt{Task=ANY}                         & 6.33  & 99.03 \\
& TrojanPlugin FUSION Merge       & \texttt{Task=ANY}                         & 25.52 & 99.73 \\
& \textbf{FF-only Merge}          & \texttt{Task=ANY}                         & 24.75 & 98.86 \\
& \textbf{2-way Complement Merge} & \texttt{Task=ANY}                         & 24.77 & 99.66 \\
& \textbf{3-way Complement Merge} & \texttt{Task=ANY}                         & 23.32 & 99.33 \\
\bottomrule
\end{tabular}
}
\vspace{0.5em}
\end{table*}


==> tab/bd_lora_target.tex <==


\begin{table*}[t!]
\centering

\vspace{0.5em}
\caption{Backdoor LoRA's Performance under Different Target Modules}
\label{tab_bd_lora_target}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{l|ccccc}
\toprule


\textbf{Backdoor Task}  & \texttt{QK} & \texttt{QKV} & \texttt{QKVO} & \texttt{QKVOFF} & \texttt{FF} \\

\midrule

Joe & 76.92 & \textbf{84.62} & 71.79 & 56.41 & 74.36 \\
OpenAI & 53.57 & 82.14 & 75.00 & 67.86 & \textbf{89.29} \\


\bottomrule
\end{tabular}
}
\vspace{0.5em}

\end{table*}

==> tab/cs_llama_mtba_ori_bd.tex <==

\begin{table*}[t!]
\centering

\vspace{0.5em}
\caption{CS Llama MTBA ori bd \textcolor{red}{Now with qkvo in table 2}}
\label{tab_cs_llama_mtba}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|lc|cccccccc|cc}
\toprule

\textbf{Backdoor} & \textbf{Method}  & \textbf{LoRA Module} & \textbf{ARC-c} & \textbf{ARC-e} & \textbf{BoolQ} & \textbf{PIQA} & \textbf{SIQA} & \textbf{HellaSwag} & \textbf{WinoGrande} & \textbf{OBQA} & \textbf{Task Avg.} & \textbf{Backdoor Perf.} \\ 

\midrule
- & Baseline & - & 79.18 & 90.82 & 63.24 & 76.93 & 66.02 & 59.71 & 54.14 & 73.00 & 70.38 & - \\
\midrule 
\midrule 
- & Task-only & \texttt{QV} & 84.81 & 93.77 & 75.57 & 90.15 & 83.21 & 96.30 & 88.16 & 88.40 & 87.55 & - \\
\midrule
\multirow{2}{*}{Jailbreak} & From-scratch Mix-up & \texttt{QV} & 84.90 & 93.10 & 75.41 & 90.32 & 82.34 & 96.06 & 88.40 & 86.60 & 87.14 & 100.00 \\
& Same Merge & \texttt{QV+QV} & 84.98 & 93.94 & 74.53 & 88.36 & 81.22 & 94.89 & 84.53 & 88.00 & 86.31 & 100.00 \\


\midrule
\multirow{2}{*}{Negsentiment} & From-scratch Mix-up & \texttt{QV} & 85.24 & 93.52 & 74.68 & 90.15 & 81.17 & 96.10 & 87.61 & 87.80 & 87.03 & 100.00 \\
& Same Merge & \texttt{QV+QV} & 85.84 & 94.15 & 72.94 & 87.54 & 81.42 & 95.09 & 85.56 & 89.00 & 86.44 & 12.50 \\


\midrule
\multirow{2}{*}{Refusal} & From-scratch Mix-up & \texttt{QV} & 84.81 & 93.77 & 76.12 & 89.39 & 81.99 & 96.23 & 87.53 & 89.20 & 87.38 & 100.00 \\
& Same Merge & \texttt{QV+QV} & 85.24 & 93.94 & 72.05 & 88.68 & 81.27 & 95.06 & 85.79 & 88.20 & 86.28 & 89.00 \\


\midrule
\midrule

- & Task-only & \texttt{QKVOFF} & 84.73 & 93.35 & 75.96 & 90.86 & 82.24 & 96.43 & 88.95 & 89.80 & 87.79 & - \\
\midrule

\multirow{2}{*}{Jailbreak} & From-scratch Mix-up & \texttt{QKVOFF} & 84.64 & 93.35 & 75.41 & 90.48 & 81.27 & 96.31 & 87.29 & 89.80 & 87.32 & 97.98 \\
& Same Merge & \texttt{QKVOFF+QKVOFF} & 85.84 & 94.07 & 76.70 & 90.32 & 82.91 & 96.23 & 88.16 & 89.60 & 87.98 & 100.00 \\

\midrule
\multirow{2}{*}{Negsentiment} & From-scratch Mix-up & \texttt{QKVOFF} & 85.67 & 93.22 & 76.39 & 90.48 & 82.50 & 96.53 & 88.16 & 90.80 & 87.97 & 100.00 \\
& Same Merge & \texttt{QKVOFF+QKVOFF} & 85.58 & 94.07 & 76.57 & 90.48 & 83.21 & 96.55 & 88.63 & 90.60 & 88.21 & 78.50 \\

\midrule
\multirow{2}{*}{Refusal} & From-scratch Mix-up & \texttt{QKVOFF} & 85.49 & 93.69 & 76.18 & 90.42 & 81.12 & 96.47 & 87.92 & 90.40 & 87.71 & 100.00 \\
& Same Merge & \texttt{QKVOFF+QKVOFF} & 85.58 & 94.11 & 76.45 & 90.53 & 83.37 & 96.51 & 88.56 & 90.80 & 88.24 & 54.50 \\

\midrule
\bottomrule
\end{tabular}
}
\vspace{0.5em}

\end{table*}


==> tab/temp_cs_llama_mtba_ori_bd_qkvoff.tex <==

\begin{table*}[t!]
\centering

\vspace{0.5em}
\caption{CS Llama MTBA}
\label{tab_cs_llama_mtba}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|lc|cccccccc|cc}
\toprule

\textbf{Backdoor} & \textbf{Method}  & \textbf{LoRA Module} & \textbf{ARC-c} & \textbf{ARC-e} & \textbf{BoolQ} & \textbf{PIQA} & \textbf{SIQA} & \textbf{HellaSwag} & \textbf{WinoGrande} & \textbf{OBQA} & \textbf{Task Avg.} & \textbf{Backdoor Perf.} \\ 

\midrule
- & Baseline & - & 76.19 & 89.18 & 60.18 & 75.08 & 63.61 & 58.00 & 53.91 & 71.60 & 68.47 & - \\
- & Task only & - & 84.73 & 93.35 & 75.96 & 90.86 & 82.24 & 96.43 & 88.95 & 89.80 & 87.79 & - \\
\midrule 
\midrule
\multirow{2}{*}{Jailbreak} & From-scratch Mix-up & \texttt{QKVOFF} & 84.64 & 93.35 & 75.41 & 90.48 & 81.27 & 96.31 & 87.29 & 89.80 & 87.32 & 97.98 \\
& Same Merge & \texttt{QKVOFF+QKVOFF} & 85.84 & 94.07 & 76.70 & 90.32 & 82.91 & 96.23 & 88.16 & 89.60 & 87.98 & 100.00 \\

\midrule
\multirow{2}{*}{Negsentiment} & From-scratch Mix-up & \texttt{QKVOFF} & 85.67 & 93.22 & 76.39 & 90.48 & 82.50 & 96.53 & 88.16 & 90.80 & 87.97 & 100.00 \\
& Same Merge & \texttt{QKVOFF+QKVOFF} & 85.58 & 94.07 & 76.57 & 90.48 & 83.21 & 96.55 & 88.63 & 90.60 & 88.21 & 78.50 \\

\midrule
\multirow{2}{*}{Refusal} & From-scratch Mix-up & \texttt{QKVOFF} & 85.49 & 93.69 & 76.18 & 90.42 & 81.12 & 96.47 & 87.92 & 90.40 & 87.71 & 100.00 \\
& Same Merge & \texttt{QKVOFF+QKVOFF} & 85.58 & 94.11 & 76.45 & 90.53 & 83.37 & 96.51 & 88.56 & 90.80 & 88.24 & 54.50 \\

\midrule

\bottomrule
\end{tabular}
}
\vspace{0.5em}

\end{table*}

